Craftax: A Lightning-Fast Benchmark for Open-Ended Reinforcement Learning

Benchmarks play a crucial role in the development and analysis of reinforcement learning (RL) algorithms. We identify that existing benchmarks used for research into open-ended learning fall into one of two categories. Either they are too slow for meaningful research to be performed without enormous computational resources, like Crafter, NetHack and Minecraft, or they are not complex enough to pose a significant challenge, like Minigrid and Procgen. To remedy this, we first present Craftax-Classic: a ground-up rewrite of Crafter in JAX that runs up to 250x faster than the Python-native original. A run of PPO using 1 billion environment interactions finishes in under an hour using only a single GPU and averages 90% of the optimal reward. To provide a more compelling challenge we present the main Craftax benchmark, a significant extension of the Crafter mechanics with elements inspired from NetHack. Solving Craftax requires deep exploration, long term planning and memory, as well as continual adaptation to novel situations as more of the world is discovered. We show that existing methods including global and episodic exploration, as well as unsupervised environment design fail to make material progress on the benchmark. We believe that Craftax can for the first time allow researchers to experiment in a complex, open-ended environment with limited computational resources.

==> olduedstuff.tex <==

% \begin{comment}
% \subsection{Unsupervised Environment Design}
% % UED results in an automatic curriculum of levels that provides a challenge for the agent in its current form. Theoretically, training on high regret levels results in the agent being more robust to unseen situations, and empirically UED results in improved generalisation~\citep{dennis2020Emergent,jiang2021Replayguided,holder2022Evolving}.
% Regret-based unsupervised environment design (UED) is a paradigm in reinforcement learning where an adversary proposes environments configurations (referred to as \textit{levels}) for an agent to learn on~\citep{dennis2020Emergent,jiang2021Replayguided,holder2022Evolving}. 
% The adversary chooses levels that maximise the agent's \textit{regret}---corresponding to the difference in performance between the optimal policy and the agent. Intuitively, levels that are too easy have a low regret, as the agent already performs well in these. Impossible levels likewise have low regret, as the optimal policy does not perform well in these. UED has been shown to result in an adaptive curriculum that improves the generalisation of agents.


% While UED is posed as a general method, it is often tested on simple environments, such as mazes and 2D car racing~\citep{dennis2020Emergent,jiang2023Minimax}, in large part because of their fast runtimes.  Since Craftax fulfills the criterion of being both fast and complex, we believe it could be a very promising domain for future research in UED.
% % One reason is that these environments are fast, and therefore allow much experimentation. However, focusing too much on these simple environments may lead to methods not being applicable more generally.
% % Since Craftax can be run very fast, and it is much more complex than, for instance, mazes, we believe it is a promising domain to benchmark  future UED research.


% \subsubsection{UED In Craftax}
% We consider \texttt{Craftax-Classic-Symbolic} and train for 1B environment steps. 
% We implement several variations of two common UED algorithms, $\text{PLR}$ and ACCEL. We also compare to Domain Randomisation (DR), which corresponds to training on randomly generated levels as normal.

% %  are generated and the agent is evaluated on these. Levels that have high regret 
% \paragraph{$\text{PLR}$}
% Prioritised level replay~\citep[PLR]{jiang2021Replayguided,jiang2020Prioritized} is a curation-based UED method which maintains a buffer of training levels .
% At every step, one of the two options is randomly chosen: (a) the agent is evaluated on randomly generated levels, and those with high regret are added to the buffer; (b) the agent is trained on a sample of high-regret levels from the buffer.
% Normal PLR performs gradient updates on the random levels, whereas robust PLR (denoted as $\text{PLR}^\perp$) only updates the agent on the levels sampled from the buffer---i.e., $\text{PLR}^\perp$ performs fewer gradient updates. This is theoretically justified and (in some domains) empirically results in higher performance~\citep{jiang2021Replayguided}.
% % The primary difference between robust PLR (denoted as $\text{PLR}^\perp$) and PLR is that the latter performs gradient updates on the random levels, whereas the former only updates the agent on the levels sampled from the buffer---i.e., robust PLR performs fewer gradient updates. This is theoretically justified and (in some domains) empirically results in higher performance~\citep{jiang2021Replayguided}.
% % works on the same basic principle as PLR. 
% % After training on levels from the buffer, these levels are randomly mutated and the high-regret levels are added to the buffer. 
% \paragraph{ACCEL}
% ACCEL~\citep{holder2022Evolving} is similar to PLR, but randomly mutates levels from the buffer, and adds the high-regret children levels to the buffer.
% ACCEL therefore increases the complexity of levels over time via iterative editing instead of having to rely solely on random generation and curation.
% ACCEL thus requires a mutation operator; here we describe three possible ways:
% % ACCEL therefore requires a mutation operator to be defined, and we describe three ways here:

% \textbf{Noise} Each level $\theta$ corresponds to the angle vectors that the perlin noise algorithm uses to generate worlds. Mutation adds a uniform random number to each element.

% \textbf{Swap} We randomly swap two different tiles. To increase relevance, one of these is within the $16\times 16$ central area of the level---close to where the agent starts.

% \textbf{Restricted Swap} To obtain more coherent levels, we restrict the tiles that can be swapped; e.g., stone can be swapped with any ore tile, and grass can be swapped with trees. %This leads to more realistic and coherent levels.
% % \begin{enumerate}
% %     \item \textit{Noise} Each level $\theta$ corresponds to the angle vectors that the perlin noise algorithm uses to generate worlds. Mutation adds a uniform random number to each element.
% %     \item \textit{Swap} We choose two different tiles, and swap their locations in the map. To make mutations more relevant, one of these tiles is within the $16\times 16$ central area of the level; i.e., close to where the agent spawns.
% %     \item \textit{Restricted Swap}  This restricts the tiles that can be swapped; for instance, stone can be swapped with any ore tile, and grass can be swapped with trees. This leads to more realistic and coherent levels.
% % \end{enumerate}

% \subsubsection{Results}
% After training for 1B timesteps, we evaluate the saved checkpoints on a fixed set of 20 evaluation levels, which were generated normally. We plot the mean and standard error over 10 independent runs.
% The primary results are presented in \cref{fig:ued:scores}. DR, PLR and $\text{PLR}^\perp$ all perform well, with PLR showing the best performance. All three ACCEL-based methods perform worse, with the swap-based ones coming in last.
% Looking at the occurrence of the individual achievements (see \cref{fig:ued:eval:all_achievements} in \cref{app:ued}) for an exhaustive list), PLR outperforms DR mainly on obtaining diamonds (\cref{fig:ued:diamonds}), one of the more difficult achievements.


% \begin{figure}[H]
%     \centering
%     \begin{subfigure}{0.47\linewidth}
%         \includegraphics[width=1\linewidth]{res/ued/plots/score.pdf}
%         \caption{Crafter Score}
%         \label{fig:ued:scores}
%     \end{subfigure}\hfill%
%     \begin{subfigure}{0.47\linewidth}
%         \includegraphics[width=1\linewidth]{res/ued/plots/diamonds.pdf}
%         \caption{Diamond Probability}
%         \label{fig:ued:diamonds}        
%     \end{subfigure}
%     \caption{Primary UED evaluation results in \texttt{Craftax-Classic}.}
% \end{figure}

% % \begin{figure}[H]
% %     \centering
% %     \begin{subfigure}{0.3\linewidth}
% %         \includegraphics[width=1\linewidth]{res/ued/replay_vs_dr/ep_lengthDR.pdf}
% %         \caption{}
% %         \label{fig:ued:length:DR}
% %     \end{subfigure}\hfill%
% %     \begin{subfigure}{0.3\linewidth}
% %         \includegraphics[width=1\linewidth]{res/ued/replay_vs_dr/ep_lengthReplay.pdf}
% %         \caption{}
% %         \label{fig:ued:length:Replay}        
% %     \end{subfigure}\hfill%
% %     \begin{subfigure}{0.3\linewidth}
% %         \includegraphics[width=1\linewidth]{res/ued/plots/eplen.pdf}
% %         \caption{}
% %         \label{fig:ued:length:eval}        
% %     \end{subfigure}
% %     \caption{Average episode length for (a) DR, (b) Replay; and (c) Evaluation levels.}
% %     \label{fig:ued:length:all}
% % \end{figure}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=1\linewidth]{res/ued/replay_vs_dr/ep_length_two.pdf}
%     \caption{Average episode length for replay and DR levels.}
%     \label{fig:ued:length:all}
% \end{figure}

% % \begin{figure}
% %     \centering
% %     \includegraphics[width=1\linewidth]{res/ued/plots/diamonds.pdf}
% %     \caption{Diamond Probability in the evaluation levels}
% %     \label{fig:ued:diamonds}
% % \end{figure}

% \paragraph{Robust vs Non-Robust PLR}
% We find that Robust PLR performs slightly worse than normal PLR, despite theoretical justification to the contrary~\citep{jiang2021Replayguided}. We believe this is due to the Craftax world generation consistently generating high-quality and solvable levels. Therefore, the agent is not penalised by training on these DR levels; to the contrary, performing only half the gradient updates (as robust PLR does) results in worse performance.

% \paragraph{Replay vs DR metrics \& Distribution Shift}
% We perform further analysis of the performance of each method during training, and consider two classes of levels separately, random (denoted as DR) and replay levels. Replay levels are those that each method actually trained on, and tend to have high regret score. We show the full results in \cref{fig:ued:replay_vs_dr} in \cref{app:ued}.
% We find that ACCEL-based methods perform differently in replay levels compared to DR. For instance, the two swap-based ACCEL methods collect diamonds nearly 80\% of the time during replay levels, but less than 10\% of the time on random levels. PLR-based methods also perform better during replay compared to DR, but not to such an extent. We also observe average episode lengths (shown in \cref{fig:ued:length:all}) is also different between replay and DR levels. The swapping ACCEL methods have episodes more than twice as long during replay compared to DR. This may indicate that the generated levels are easier, so the agent dies less, and therefore spends more time on collecting achievements.
% % Overall, we can make several observations:
% % \begin{enumerate}
% %     \item The performance on replay levels is significantly different to the DR performance for ACCEL-based methods. In particular, the two swap-based ACCEL methods collect diamonds nearly 80\% of the time during replay levels, but less than 10\% of the time on random levels.
% %     \item Based on replay performance, ACCEL-based methods outperform PLR-based methods (of course, this is somewhat unfair, as the replay distributions are not the same). DR performance, however, is vastly different and ACCEL-based methods perform worse.
% %     \item The average episode lengths (shown in \cref{fig:ued:length:all}) is also different between replay and DR levels. The swapping ACCEL methods have episodes more than twice as long during replay compared to DR. This may indicate that the generated levels are easier, so the agent dies less, and can spend more time on collecting achievements.
% % \end{enumerate}


% This is an instantiation of the curriculum-induced covariate shift problem identified by \citet{jiang2022Grounding}. In particular, UED methods may shift the distribution of training levels to something different to the ground truth distribution (which is DR in this case). 
% In theory, this only matters if this curriculum shift changes certain unobserved properties of the environment. However, here we empirically show this problem occurs even when the agent can observe much of the environment. This is due to the agent performing a significant amount of training on levels from a different distribution to what it is evaluated on, and therefore not perfomring as well as it could have.

% One possible reason is that these levels provide a higher score---as the agent, for instance, can more easily obtain all achievements.
% This results in its regret score being high on these, and the adversary continues to sample these levels. This is despite these levels not being as useful for generalising to the default (DR) distribution over levels. 
% % We also note that the average episode length of ACCEL-swap is three times longer in replay (1500) compared to DR (500). This may indicate that the generated levels are easier, so the agent dies less, and can spend more time on collecting achievements.


% % \cref{fig:replay_vs_dr} shows that during replay, ACCEL methods obtain diamonds more than 80\% of the time, but this does not transfer to DR levels.
% \subsubsection{Qualitative Results}
% We provide several figures and analyses of the levels generated by each method.
% \cref{fig:examples_accel_noise,fig:examples_accel_swap,fig:examples_accel_swap_restrict,,fig:examples_normal_plr,fig:examples_robust_plr,fig:examples_dr} in \cref{app:ued} show these levels. The curation-based methods generally cause resources to be more centrally-located, near where the player spawns. The unrestricted ACCEL swapping method generates levels that are visually very different to the normally generated ones, as there is no restriction to where it can place tiles. The restricted swapping method generates plausible levels, and so does the noise-based method.



% \subsubsection{Summary}
% In conclusion, we demonstrate that we can apply existing UED methods to Craftax, and that PLR outperforms DR, especially on harder achievements. We have further shown that, despite theoretical justification, robust PLR underperforms normal PLR. Furthermore, using ACCEL may cause the agent to perform well on the replay distribution of levels, but fail to generalise to the normally-generated levels. Craftax therefore challenges current UED methods, and can be used as a more challenging domain on which to develop future UED algorithms on.

% \end{comment}

